StableSemantics: A Synthetic Language-Vision Dataset of Semantic Representations in Naturalistic Images

Understanding the semantics of visual scenes is a fundamental challenge in Computer Vision. A key aspect of this challenge is that objects sharing similar semantic meanings or functions can exhibit striking visual differences, making accurate identification and categorization difficult. Recent advancements in text-to-image frameworks have led to models that implicitly capture natural scene statistics. These frameworks account for the visual variability of objects, as well as complex object co-occurrences and sources of noise such as diverse lighting conditions. By leveraging large-scale datasets and cross-attention conditioning, these models generate detailed and contextually rich scene representations. This capability opens new avenues for improving object recognition and scene understanding in varied and challenging environments. Our work presents StableSemantics, a dataset comprising 224 thousand human-curated prompts, processed natural language captions, over 2 million synthetic images, and 10 million attention maps corresponding to individual noun chunks. We explicitly leverage human-generated prompts that correspond to visually interesting stable diffusion generations, provide 10 generations per phrase, and extract cross-attention maps for each image. We explore the semantic distribution of generated images, examine the distribution of objects within images, and benchmark captioning and open vocabulary segmentation methods on our data. To the best of our knowledge, we are the first to release a diffusion dataset with semantic attributions. We expect our proposed dataset to catalyze advances in visual semantic understanding and provide a foundation for developing more sophisticated and effective visual models. Website: https://stablesemantics.github.io/StableSemantics

==> fig_text/cluster_text.tex <==
\begin{figure}[h]
  \centering
\includegraphics[width=0.8\linewidth]{fig_pdf/clusters.pdf}
   \vspace{-1mm}
  \caption{\textbf{Clustering within the food ROI and within OPA}. Clustering of encoder model weights for each region is shown for two example subjects on an inflated cortical surface. 
  % Food clusters reveal alternating patches, with one cluster located more medially. 
  % We find the 2nd food cluster to show more high saturation preference. OPA is consistently split into anterior-posterior in all four subjects. With the anterior showing an outdoor preference.
  }
  \vspace{-0.2cm}
  \label{fig:cluster}
\end{figure}

==> sections/06_Acknowledgements.tex <==
\section{Acknowledgements} This work used Bridges-2 at Pittsburgh Supercomputing Center through allocation SOC220017 from the Advanced Cyberinfrastructure Coordination Ecosystem: Services \& Support (ACCESS) program, which is supported by National Science Foundation grants \#2138259, \#2138286, \#2138307, \#2137603, and \#2138296. We also thank the Carnegie Mellon University Neuroscience Institute for support.
